Direct Measurement of the Forbidden $2^{3\!}S_1 \rightarrow 3^{3\!}S_1$ Atomic Transition in Helium

We present the detection of the highly forbidden $2^{3\!}S_1 \rightarrow 3^{3\!}S_1$ atomic transition in helium, the weakest transition observed in any neutral atom. Our measurements of the transition frequency, upper state lifetime, and transition strength agree well with published theoretical values, and can lead to tests of both QED contributions and different QED frameworks. To measure such a weak transition, we developed two methods using ultracold metastable ($2^{3\!}S_1$) helium atoms: low background direct detection of excited then decayed atoms for sensitive measurement of the transition frequency and lifetime; and a pulsed atom laser heating measurement for determining the transition strength. These methods could possibly be applied to other atoms, providing new tools in the search for ultra-weak transitions and precision metrology.

==> latexmkrc <==
$ENV{'TEXINPUTS'}='./tex//:' . $ENV{'TEXINPUTS'};
$ENV{'BSTINPUTS'}='./bst//:' . $ENV{'BSTINPUTS'};

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
